Primal-Dual Gradient Methods for Searching Network Equilibria in Combined Models with Nested Choice Structure and Capacity Constraints

We consider a network equilibrium model (i.e. a combined model), which was proposed as an alternative to the classic four-step approach for travel forecasting in transportation networks. This model can be formulated as a convex minimization program. We extend the combined model to the case of the stable dynamics (SD) model in the traffic assignment stage, which imposes strict capacity constraints in the network. We propose a way to solve corresponding dual optimization problems with accelerated gradient methods and give theoretical guarantees of their convergence. We conducted numerical experiments with considered optimization methods on Moscow and Berlin networks.

==> images/dgap.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Computational time, minutes},
xmajorgrids,
xmin=-13.4554691982269, xmax=292.942112782796,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Duality gap},
ymajorgrids,
ymin=16.2760740503718, ymax=1237437954684.13,
ymode=log,
ytick style={color=black},
ytick={0.1,10,1000,100000,10000000,1000000000,100000000000,10000000000000,1e+15},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{3}}\),
  \(\displaystyle {10^{5}}\),
  \(\displaystyle {10^{7}}\),
  \(\displaystyle {10^{9}}\),
  \(\displaystyle {10^{11}}\),
  \(\displaystyle {10^{13}}\),
  \(\displaystyle {10^{15}}\)
}
]
\addplot [draw=mediumpurple148103189, fill=mediumpurple148103189, forget plot, mark=*, only marks]
table{%
x  y
0.471693619092306 1176354995.68263
7.55967458486557 4064995.51580358
14.7971276919047 1585729.04284006
21.7634329756101 891150.07864368
28.8247673392296 523434.456741542
35.7299989064535 321669.591877162
42.4836260676384 200750.91682139
49.3870165944099 131401.979270428
56.2620198090871 84902.39286533
63.0469854156176 57394.4624097645
69.8985745112101 39323.212123543
76.7445380210876 27514.1052582562
83.5337691863378 19689.2090221941
90.4024851640065 14507.2062773407
97.2295503576597 10464.6857132912
104.1484866937 7595.18758064508
110.937427731355 5446.2186717391
117.81846101284 3894.27477356791
124.719880370299 2827.35742974281
131.585482128461 2092.80059784651
138.411969459057 1530.43873143196
145.416398104032 1117.35138463974
152.393862513701 854.63518217206
159.45637794733 619.432425528765
166.453763552507 465.618164360523
173.492432240645 376.346700906754
180.484850537777 294.265100419521
187.588025180499 222.953204631805
194.521945412954 203.018495708704
201.507578202089 156.878733366728
208.520057038466 126.515051782131
215.565074249109 100.597166180611
222.510572270552 111.672351688147
229.546884961923 80.577468931675
236.437541778882 83.044261097908
243.511394937833 67.4200243353844
250.488455001513 69.9230303764343
257.50273570617 63.3922297954559
264.562016920249 63.1105737686157
271.583381088575 61.7045949697495
278.749624379476 50.8322547674179
};
\addplot [draw=forestgreen4416044, fill=forestgreen4416044, forget plot, mark=*, only marks]
table{%
x  y
0.548119421799978 5875743753.99046
6.00118607680003 980963.229369551
11.4539016405741 277983.339598775
16.8048702398936 177897.7007429
22.1947771430016 75936.3325298429
27.5889187256495 48539.4376375079
33.0104064742724 42985.7875972986
38.4309130311012 25806.5717770159
43.722837348779 27803.618073225
49.0722175637881 20417.4860777855
54.5774902025859 18383.7867866755
59.902151564757 10947.3854076862
65.4121315519015 9911.59916585684
70.8481623649597 10974.2160077095
76.3018157641093 7173.17895165086
81.6555424928665 8144.66339558363
87.0246085127195 6496.01973506808
92.3705481052399 5337.77261412144
97.8340717673302 4558.38003465533
103.182754679521 4927.77484762669
108.519647026062 5717.91028141975
113.946590387821 4067.71149680018
119.38849149545 4465.55908066034
124.720185093085 4146.11317282915
130.182063853741 3353.49835327268
135.669336064657 3051.71932783723
141.130463512739 4438.3955655694
146.632810016473 2976.41015279293
152.136308193207 2607.81742343307
157.743713156382 4069.99052342772
163.370520039399 2875.25663805008
168.925697267056 3127.62191012502
174.462250820796 2458.11233451962
179.932447405656 2221.42169591784
185.4546910127 2104.38147431612
191.049272286892 2033.56163275242
196.576691905657 2182.82015743852
202.014765036106 2695.52364838123
207.476763260365 2145.3665882647
213.115786643823 2124.75556835532
218.604920514425 2469.96909564734
224.208601566156 1660.06970509887
229.741024148464 2036.61866599321
235.247555947304 1497.72520342469
240.807710679372 1808.03983017802
246.313227609793 1334.73918789625
251.931732535362 2205.62427544594
257.533929363887 1398.32355493307
263.118235385418 1442.49159422517
268.788958740234 1187.18705144525
273.974786543846 1210.69226449728
};
\addplot [draw=steelblue31119180, fill=steelblue31119180, forget plot, mark=*, only marks]
table{%
x  y
11.5320949077606 72426787.2533198
23.5118829488754 396217556654.384
35.2977201541265 5452280.47472209
46.9245350321134 802400.861786544
58.5613099098206 205698.744781137
70.1918295741081 162956.572669506
81.8107367197672 160616.842041254
93.4353009025256 198833.58210519
105.044639201959 269297.754647523
116.645345199108 245449.742302656
128.245223712921 246574.59068504
139.877738114198 285763.648211926
151.499468004704 280648.226726979
163.129851229986 225973.641916215
174.715938270092 241942.166892439
186.34846735398 260583.513394833
197.933357576529 295994.299571753
209.518978397051 302998.10830605
221.095550600688 249108.879304975
232.690443181992 250455.372579992
244.264173777898 230995.492960185
255.845887549718 263146.014268875
267.421058452129 245631.978812397
279.014949965477 259248.605973214
};
\addplot [semithick, mediumpurple148103189]
table {%
0.471693619092306 1176354995.68263
7.55967458486557 4064995.51580358
14.7971276919047 1585729.04284006
21.7634329756101 891150.07864368
28.8247673392296 523434.456741542
35.7299989064535 321669.591877162
42.4836260676384 200750.91682139
49.3870165944099 131401.979270428
56.2620198090871 84902.39286533
63.0469854156176 57394.4624097645
69.8985745112101 39323.212123543
76.7445380210876 27514.1052582562
83.5337691863378 19689.2090221941
90.4024851640065 14507.2062773407
97.2295503576597 10464.6857132912
104.1484866937 7595.18758064508
110.937427731355 5446.2186717391
117.81846101284 3894.27477356791
124.719880370299 2827.35742974281
131.585482128461 2092.80059784651
138.411969459057 1530.43873143196
145.416398104032 1117.35138463974
152.393862513701 854.63518217206
159.45637794733 619.432425528765
166.453763552507 465.618164360523
173.492432240645 376.346700906754
180.484850537777 294.265100419521
187.588025180499 222.953204631805
194.521945412954 203.018495708704
201.507578202089 156.878733366728
208.520057038466 126.515051782131
215.565074249109 100.597166180611
222.510572270552 111.672351688147
229.546884961923 80.577468931675
236.437541778882 83.044261097908
243.511394937833 67.4200243353844
250.488455001513 69.9230303764343
257.50273570617 63.3922297954559
264.562016920249 63.1105737686157
271.583381088575 61.7045949697495
278.749624379476 50.8322547674179
};
\addlegendentry{USTM}
\addplot [semithick, forestgreen4416044]
table {%
0.548119421799978 5875743753.99046
6.00118607680003 980963.229369551
11.4539016405741 277983.339598775
16.8048702398936 177897.7007429
22.1947771430016 75936.3325298429
27.5889187256495 48539.4376375079
33.0104064742724 42985.7875972986
38.4309130311012 25806.5717770159
43.722837348779 27803.618073225
49.0722175637881 20417.4860777855
54.5774902025859 18383.7867866755
59.902151564757 10947.3854076862
65.4121315519015 9911.59916585684
70.8481623649597 10974.2160077095
76.3018157641093 7173.17895165086
81.6555424928665 8144.66339558363
87.0246085127195 6496.01973506808
92.3705481052399 5337.77261412144
97.8340717673302 4558.38003465533
103.182754679521 4927.77484762669
108.519647026062 5717.91028141975
113.946590387821 4067.71149680018
119.38849149545 4465.55908066034
124.720185093085 4146.11317282915
130.182063853741 3353.49835327268
135.669336064657 3051.71932783723
141.130463512739 4438.3955655694
146.632810016473 2976.41015279293
152.136308193207 2607.81742343307
157.743713156382 4069.99052342772
163.370520039399 2875.25663805008
168.925697267056 3127.62191012502
174.462250820796 2458.11233451962
179.932447405656 2221.42169591784
185.4546910127 2104.38147431612
191.049272286892 2033.56163275242
196.576691905657 2182.82015743852
202.014765036106 2695.52364838123
207.476763260365 2145.3665882647
213.115786643823 2124.75556835532
218.604920514425 2469.96909564734
224.208601566156 1660.06970509887
229.741024148464 2036.61866599321
235.247555947304 1497.72520342469
240.807710679372 1808.03983017802
246.313227609793 1334.73918789625
251.931732535362 2205.62427544594
257.533929363887 1398.32355493307
263.118235385418 1442.49159422517
268.788958740234 1187.18705144525
273.974786543846 1210.69226449728
};
\addlegendentry{Evans algorithm}
\addplot [semithick, steelblue31119180]
table {%
11.5320949077606 72426787.2533198
23.5118829488754 396217556654.384
35.2977201541265 5452280.47472209
46.9245350321134 802400.861786544
58.5613099098206 205698.744781137
70.1918295741081 162956.572669506
81.8107367197672 160616.842041254
93.4353009025256 198833.58210519
105.044639201959 269297.754647523
116.645345199108 245449.742302656
128.245223712921 246574.59068504
139.877738114198 285763.648211926
151.499468004704 280648.226726979
163.129851229986 225973.641916215
174.715938270092 241942.166892439
186.34846735398 260583.513394833
197.933357576529 295994.299571753
209.518978397051 302998.10830605
221.095550600688 249108.879304975
232.690443181992 250455.372579992
244.264173777898 230995.492960185
255.845887549718 263146.014268875
267.421058452129 245631.978812397
279.014949965477 259248.605973214
};
\addlegendentry{Four-step procedure}
\end{axis}

\end{tikzpicture}

